A Blueprint for Interoperable Blockchains

Research in blockchain systems has mainly focused on improving security and bridging the performance gaps between blockchains and databases. Despite many promising results, we observe a worrying trend that the blockchain landscape is fragmented in which many systems exist in silos. Apart from a handful of general-purpose blockchains, such as Ethereum or Hyperledger Fabric, there are hundreds of others designed for specific applications and typically do not talk to each other. In this paper, we describe our vision of interoperable blockchains. We argue that supporting interaction among different blockchains requires overcoming challenges that go beyond data standardization. The underlying problem is to allow smart contracts running in different blockchains to communicate. We discuss three open problems: access control, general cross-chain transactions, and cross-chain communication. We describe partial solutions to some of these problems in the literature. Finally, we propose a novel design to overcome these challenges.

==> sec/analysis.tex <==
We obtained 72 hours Internet traffic log from our university firewall to
identify the frequency of users logging into common servers in the internet. We
analyzed the access pattern of 2512 users to 182,600 public servers running a
service on port 443.  However, we did not consider all the public servers as
many of them were not frequently accessed by majority of users (for the current
study we defined the threshold of minimum of 50 unique user access for a server
to be considered). 

\begin{figure}[t!]
    \centering  
    \def\svgwidth{\columnwidth}
    \input{fig/aaf.pdf_tex}
    \caption{Average of access frequencies of servers in different tiers.}
    \label{fig:aaf}
\end{figure}

We sampled the selected servers into different tiers based on the number of
unique users accessed it over the 72 hours (stratified sampling). The tier 1
with more than 1600 users, tier 2 with 800 users, tier 3 with 400 users, tier 4
with 200 users and remaining users into tier 1.  The average of time difference
between consecutive user accesses (known as access frequency) to individual
servers in each tiers were measured. We can see that servers in higher tier
(tier 1\&2) has higher access frequency with a mean access frequency of 10
seconds (ie an authentication happens every 10 seconds on average). The
cumulative distribution function (CDF) of lognormal distribution of average
access frequency to servers in each tier is plotted in
~\autoref{fig:tier1},~\autoref{fig:tier2},~\autoref{fig:tier3}, and
~\autoref{fig:tier4}.


\subsection{Survey}

In order to understand the frequency of user login we conducted a small survey
on 75 users majority of whom were university students. To get a clear picture, we
asked them specific questions on their authentication activity on email, social
media and online shopping unlike other studies which consider other mean of
authentications such as unlocking a phone or laptop or opening a house door.

All the 75 users were using email in their daily life, however, most of them
don't authenticate everyday with their username and password as they save their
cookies in the browser. Around 13\% of the users responded that they used their
email from their phone which reduces the frequency of authentication with
entering username and password (without using cookie or other authentication
tokens).  

This study helps us to understand that majority around 80\% of the users don't
clear their cookies especially while using their local computers and add their
smartphone as trusted device.   

==> sec/details.tex <==
\subsection{Initialization}
The first step that a client takes to join the system is to register its
identity. In order to accomplish it, the client first generates its
public/private keypair $(pk,sk)$ and generates a larger random number $cnt$
as its initial \textit{authentication counter}.

Afterwards, the clients creates the following \textit{registration request}
\begin{equation} \label{eq:reg}
    REGISTER, pk, meta, tkn, \sigma,
\end{equation}
where $meta$ is identity metadata (e.g., a human-readable name or contact
information), $tkn=H(VRF_{sk}(cnt))$ and is called an \textit{authentication
token}, and $\sigma$ is a client's signature computed over the message, i.e.,
$\sigma=Sign_{sk}(REGISTER\|pk\|meta\|tkn)$.\footnote{For a simple description, we
assume that the clients uses the same keypair in different cryptographic
constructions (like VRF, digital signatures, etc...) In practice, different
cryptographic primitives may require different keypairs.} The request is sent to
any entity able to write to the blockchain.

Upon receiving the request, the receiver validates it by verifying its
signature.  Afterwards, the receiver registers the identity by a) inserting the
key-value pair $(pk, meta)$ into the \textit{identities map} of the blockchain,
and b) inserting the token $tkn$ into the \textit{tokens set} store
on the blockchain.  When values are added, the receiver returns to the client
proofs $\pi_{id}$ and $\pi_{tkn}$ that respectively prove that the client's
identity and the token were added to the blockchain.
After receiving and validating the proofs, the client increments its counter by
one and is ready to use its blockchain identity for authentication.
\psz{these proofs are not necessary, but may be helpful}

\begin{figure}[t!]
    \centering  
    \def\svgwidth{\columnwidth}
    \input{fig/Architecture.pdf_tex}
    \caption{Highlevel Overview}
    \label{fig:architecture}
\end{figure}

\begin{figure}[t!]
    \centering  
    \def\svgwidth{\columnwidth}
    \input{fig/identity_map.pdf_tex}
    \caption{Identity and Token Map}
    \label{fig:identity}
\end{figure}

\subsection{Authentication Process}
The authentication process is conducted between a client and an
\textit{authentication service} and is  a core element of our protocol.
The goal of the process is to convince the authentication service to authenticate
the client, more specifically, to ensure that:
\begin{itemize}
    \item the requester possesses the $sk$ corresponding to the client's
        identity at the time of the authentication process,
    \item the client's identity is registered with the blockchain,
    \item the authentication process is \textit{consistent} with the previous
        authentication of this client.
\end{itemize}
The first condition it quite standard for authentication protocols. The
second is to make the blockchain an identity provider for the clients.
The last condition guarantees both the client and the service, that the client
is aware of its latest authentication.

To initiate the process, the clients sends the following
\textit{authentication request} to the service:
\begin{equation} \label{eq:auth}
    AUTH, pk, \pi_{id}, \pi_{tkn_{-1}} cnt, v_{-1}, v,
\end{equation}
where $v_{-1} = VRF_{sk}(cnt-1)$ and $v=VRF_{sk}(cnt)$.
The service validates the message:
\begin{enumerate}
    \item verifying that the values $v_{-1}$ and $v$ are authentically generated
        by the client for the inputs $cnt-1$ and $cnt$, correspondingly,
    \item the identity presence proof $\pi_{id}$ is correct and corresponds to
        $pk$,
    \item the token presence proof $\pi_{tkn_{-1}}$ corresponds to the
        authentication token of value $H(v_{-1})$,
    \item and the authentication token $H(v)$ is not registered in the
        blockchain.
\end{enumerate}
For the last check, the service needs to contact the blockchain platform (or
lookup it if the service caches the blockchain already) and obtain a proof that
$H(v)$ was not appended to the blockchain's tokens set.
With these checks the service gets confident that the client's previous token
was used and the current one was not used yet.

After these steps, the next phase is actual authentication.
We do not specify how the client proves its possession of $sk$ and our system
can be combined with existing and widely deployed systems~\cite{}.
We emphasize, however, that the authentication process should protect the
initial message from \autoref{eq:auth}.
\psz{do we want to give some exact protocol? it?}
\psz{@ZP can we use something password-based, in general?}

\zli{TBD, password authentication ...
The problem is that if the private key for the transactions is password derived (for easy remembrance), there is a risk of brute force attacks either by a malicious service or any adversary who views the transaction from a password derived wallet to a multi-sign smart contract on the public blockchain.
}





After the successful authentication, the service submits  to the blockchain the
following data:
\begin{equation}\label{eq:data}
    tkn, log,
\end{equation}
where $tkn$ is the client's current
token $H(v)$ and $log=Enc_{pk}(info)$.
The latter message, is a ciphertext in which the service encrypts information
about the authentication process (like the service name). This ciphertext allows
the client to audit its entries in the blockchain.
For anonymity reasons, submission of the token by the service provider is
anonymized. We use... \psz{@ZP...}\zli{TBD}
After the token is inserted to the tokens set, the
service returns to the client a proof $\pi_{tkn}$ stating it.
The client receives the proof, increments the counter, and can start using the
service.


\subsection{Blockchain Design}
So far we assumed two abstract data structures, i.e., the identity map and the
tokens set, that are essential for our blockchain functionality.
We assume that the blockchain stores a list of all transactions received, but to
facilitate operations requires from our data structures, we enrich this simple
blockchain design.
In our system we introduce the two following data structures:
Identities tree...
Tokens tree...

Both trees are based upon a Merkle hash tree. We sort leaves of these trees in
lexicographical order...

figures...

\subsection{Audit}




==> sec/implementation.tex <==
https://github.com/google/trillian


==> sec/overview.tex <==
\subsection{Problem Definition}
\label{subsec:system_model}
Our system consists of three types of entities: {\em clients},  {\em identity providers}, and {\em service
providers}. The clients have unique identities assigned to them by some {\em identity providers} in the form
of user credentials. When the client wishes to use some resources, it contacts the corresponding service
provider and starts an authentication protocol, which we refer to as a {\em login} protocol. Our goal is to
design and implement an authentication system with the following security properties:  

\begin{itemize}
    \item {\bf Authentication:} the service provider can authenticate clients securely.
    \item {\bf Login transparency:} the client can verify the complete history of its login. 
    \item {\bf Privacy:} adversaries cannot learn about any login involving honest client and service
    provider. 
    \item {\bf Scalability:} the system supports a large number of users with comparable latencies to today's
    authentication system.     
\end{itemize}

We note that login transparency is the distinguishing property of our system compared to other authentication
system. It allows the client to check when and to which services its credentials have been used for successful
authentication. More importantly, the client can detect if there have been unauthorized logins with his
credentials.  

\subsubsection*{Threat model}
The client is trusted, but an adversary can steal its credentials to login to a trusted service provider.
This can be done by exploiting vulnerabilities at the client's software that store or use the credentials. We
note that stealing credentials is a practical and significant threat, especially when the credentials are used
to access financial services. 


The identity provider is semi-honest. It is trusted with respect to granting and attesting to the correct
client credentials. But it is curious, in the sense that it wants to learn which client login to which service
provider and at which time. But we assume the communication between the client and service provider is secure,
and no timing information is leaked to other entities. 

A service provider can be compromised by the adversary. Such the malicious service provider can deviate
arbitrarily from the protocol, and it can make use the stolen credentials. When not compromised, the service
provider is semi-host, that is, it follows the login protocol correctly, but it wants to learn information
other than what the login protocol reveals. Like the identity provider, it wants to learn which client login
to which (other) services.  

\subsection{Challenges and Approaches}
\label{subsec:challenges}
Ideas/Insights: 
1) use blockchain as a identity provider
2) provide security properties that the current systems cannot provide


\subsection{Protocol Overview}
\label{subsec:protocol_overview}

A high level description is presented in \autoref{fig:overview}.
\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/overview}
  \caption{A high-level overview of the protocol.}
  \label{fig:overview}
\end{figure*}

In short, the protocol can be described in the following steps:

\psz{rewrite}
\begin{enumerate}

    \item The client $c$ joins the system
    \begin{enumerate}
        \item Generates a public/private keypair $(pk_c,sk_c)$, and
        \item Generates a long ordered list of large random numbers, called
            \textit{login values}, and aggregates them into a Merkle-tree-based
            accumulator with the root value $r_c$.
    \end{enumerate}

    \item The client registers its \textit{identity record} with the blockchain
        by submitting a transaction including
        \begin{equation}\label{eq:id}
            c, pk_c, r_c
        \end{equation}
        (note that no login value can be derived from the root value $r_c$).

    \item Whenever the client wishes to authenticate to the service $s$ she
        proves to $s$ that
        \begin{enumerate}
            \item her identity record (see \autoref{eq:id}) is
                indeed in the blockchain,
            \item she possesses the secret key ($sk_c$) corresponding to the
                private key $pk_c$,
            \item she knows the next ($i$th) unused login value $v^i_c$ (the
                value is revealed to the service).
        \end{enumerate}

     \item After successfully validating the received statements, the service
         authenticates the client and publishes the following message at the
         blockchain
        \begin{equation}\label{eq:record}
            v^i_c, Enc_{pk_c}(s).
        \end{equation}
        \psz{AFAIR we wanted to encrypt something more here, what was that? I'm
        not sure whether encrypting $s$ identity makes sense, as probably it
        would be revealed by putting the transactions to the blockchain (i.e.,
        layer below). Would be nice to give some privacy to that --
        ring/threshold/anonymous signatures?\\
        Do we want to prove that $sk_c$ was indeed used? Then we could require
        some singature of $(v^i_c, nonce)$ put into the encryption above}

     \item At any point in time, the client can easily audit the blockchain by
         checking whether her next login value $v^{i+1}_c$ is in the blockchain
         -- that would imply that her credentials were used unauthorized. 
\end{enumerate}
\psz{side thought: another point is that it could be implementing 2FA natively}



==> sec/pre.tex <==
\subsection{Decentralized Identity}
\bithu{There are some additional text included, added as notes will remove it later.}

The conventional identity management systems are based on a central authority.
These central authorities serve as a root of trust which make it extremely
difficult for users to control their own identity. In order to address this,
Decentralized Identity (DID)~\cite{did} was purposed, in which the identity is
owned and controlled by the entity which created it. Each DID is associated with
a DID document also known as DID descriptor object (DDO).   

\begin{equation}
    \textbf{did:btcx:123456789abcdefghijk}
    \label{eq1}
\end{equation}

Example ~\ref{eq1} represent a DID which is globally unique and consist of three
parts. First, \textit{did} is the URL schema, then \textit{btcx} is the DID
method and last \textit{123456789abcdefghijk} is a method specific identifier. A
DID comes with some additional properties which its predecessor identifiers
(UUID and URI) doesn't provide such as 1) persistent (URI provides persistence,
however, depends on central authority), 2) decentralized, 3) dereference-able,
and 4) cryptographically verifiable. A DID resolves to a DID Document which is a
JSON data structure containing meta data describing an identity owner including
the cryptographic key material required for the identity owner to prove
ownership and control of the DID document. A DID method define a specific DID
scheme which can be implemented on a specific distributed ledger or network,
including the precise method by which DID and DDOs can be read, written and
revoked. In the above example DID, the DID is registered onto Bitcoin
Blockchain. 

There are many other DID methods, including those which are not related to a
blockchain such as "git" DID Method which use Git repository as a source of
truth about the repository identity and its contributor's identity. Another
motivation for "git" DID method is to encourage contributions to DID spec which
allow rapid development of extensions to these without the use of slow or
complicated trustless infrastructure such as Blockchain or Distributed
System~\cite{gitdid}. So here we trust GitHub to manage DDOs. The basic idea is
to resolve a DID Document to a GitHub repository and then check the signature
for the same to cryptographically validate the DDO document to make sure that it
indeed belong to the entity which owns it. The purpose of DDO is to specify the
public key, authentication protocol, and service endpoint necessary to bootstrap
cryptographically verifiable interaction with the entity associated with the
identity.

\subsubsection{DID Auth Protocol}

Implementation of TLS using public key associated with a DID rather than X.509
Certificate. It allows two DID owners to be able to mutually authenticate with a
high degree of certainty and can establish an ephemeral, secure communication
channel. Slight modification needed in TLS libraries to implement DID-TLS which
is not yet completed.

\subsubsection{SideTree Protocol}
SideTree~\cite{sidetree} allow for efficient interaction with the blockchain
during a DID resolve operation. They batch the DID document and then anchor it
onto the Blockchain rather than writing each DID resolve operation onto to the
blockchain. ION~\cite{ion} is a DID Method implementation using the SideTree
protocol on top of Bitcoin to support DIDs/DPKI at scale. ION make it possible
to anchor tens of thousands of DID/DPKI operation on a target blockchain using a
single on-chain transaction.    


Attacker Model -> (adv colluding with service doesn't have to compromise
clients)
Assumptions

% The notation used throughout the paper is presented in \autoref{tab:notation}
% \begin{table}[h!]
% \begin{center}
% % \renewcommand*{\arraystretch}{1.25}
%     \begin{tabular}{ll}
% $\{msg\}_A$ & denotes the message $msg$ digitally signed by $A$, \\
% $h(.)$ & is a cryptographic hash function, \\
% $\|$ & is the string concatenation, \\
% $r\xleftarrow{R}S$ & denotes that $r$ is an element randomly selected from the set $S$,\\
% $\{0,1\}^n$ & is a set of all $n$-bit long strings,\\
% $t_x$ & is a Unix timestamp expressed in seconds. \\
% \end{tabular}
% \end{center}
%     \caption{Notation used throughout the paper.}
%     \label{tab:notation}
% \end{table}


==> sec/related-sign.tex <==



\subsection{Related Group Signature and Ring Signature}
\zli{TBD, I am working this part.}


\noindent\textbf{Group Signature}.
Group signature, introduced by Chaum and van Heyst~\cite{XXXX}, is a fundamental
anonymity primitive which allows any member of the group can sign messages on behalf of the whole group (i.e., provide anonymity for signers), but the resulting signature keeps the identity of the signer secret.

\noindent\textbf{Ring Signature}.
Ring signatures are a type of cryptographic digital signature and were actually invented back in 2001 by Ron Rivest, Adi Shamir, and Yael Tauman and subsequently introduced at Asiacrypt. The concept is similar to that of group signatures, however, there is no way to identify the actual signer of a ring signature transaction and an arbitrary group of users can be included in the ring signature without any additional setup. However, ring signatures take the concept of group signatures further to provide better privacy for the user. In a P2P transaction format as is the case with cryptocurrencies, specifically using the CryptoNote coins as a reference, ring signatures protect the sender by obscuring the input side of a transaction so that it is computationally infeasible to determine who the actual signer of a transaction is.



\noindent\textbf{Existing Schemes}
\zli{TBD}




\noindent\textbf{Relationships with Zero-Knowledge Proof}
\zli{TBD}


\noindent\textbf{Why we use Group or Ring Signature?}
\zli{TBD}



\section{Cryptographic Tools or Building Blocks}
\zli{These formal definitions of syntax, correctness and security requirements could move to Appendix.}
\subsection{(Non-Interactive) Zero-Knowledge Proof System}


we recall a standard definition of non-interactive zero-knowledge proof systems. Let $\cal{L}_{\cal{R}}$ be an NP-language with witness relation $\cal{R}$: $\mathcal{L}_{\mathcal{R}}=\{ x  | \exists  w: \mathcal{R}(x, w)=1\}$. A noninteractive proof system $\Pi_{ZK}$ consists of the following polynomial-time algorithms (PPT) algorithms

\begin{itemize}
  \item $crs\gets Setup(1^{\lambda})$ Takes a security parameter $\lambda$ as input, and outputs a common reference string $crs$.
  \item $Proof(crs, x, w)$: Takes a common reference string $crs$, a statement $x$, and a witness $w$ as input, and outputs a proof $\pi$.
  \item $Vrfy(crs, x, \pi)$: Takes a common reference string $crs$, a statement $x$, and a proof $pi$ as input, and outputs a bit $b\in \set{0,1}$.
\end{itemize}
We require proof systems to be complete, sound, and zero-knowledge. The detailed definitions are omitted here.
\zli{Extend to Signatures of Knowledge???}



\subsection{Ring Signature}

\zli{Question: can we require a trust party or manager? If no, we need to consider ring signature rather than group signature.}

\zli{https://eprint.iacr.org/2018/728.pdf}

Ring signatures were invented by Ron Rivest, Adi Shamir, and Yael Tauman, and introduced at ASIACRYPT in 2001. Importantly, ring signature allows a signer to leak secrets anonymously, without the risk of identity escrow. At the same time, the ring signature provides great flexibility: No group manager, no special setup, and the dynamics of group choice. The ring signature is, however, vulnerable to malicious or irresponsible signers in some applications, because of its anonymity.





%The name, ring signature, comes from the ring-like structure of the signature algorithm. The concept is similar to that of group signatures, however, there is no way to identify the actual signer of a ring signature transaction and an arbitrary group of users can be included in the ring signature without any additional setup.


%In a nutshell, a ring signature is a type of digital signature that can be performed by any member of a group of users that each have keys. Therefore, a message signed with a ring signature is endorsed by someone in a particular group of people.
%
%
%One of the security properties of a ring signature is that it should be computationally infeasible to determine which of the group members' keys was used to produce the signature.
%
%
%Ring signatures are similar to group signatures but differ in two key ways: first, there is no way to revoke the anonymity of an individual signature, and second, any group of users can be used as a group without additional setup.






\zli{Ring signatures take the concept of group signatures further to provide better privacy for the user. In a P2P transaction format as is the case with cryptocurrencies, specifically using the CryptoNote coins as a reference, ring signatures protect the sender by obscuring the input side of a transaction so that it is computationally infeasible to determine who the actual signer of a transaction is.}

\href{https://blockonomi.com/ring-signatures}{https://blockonomi.com/ring-signatures}


\zli{Differences between ring-Sign and group-sign}


Ring signature is a primitive which provides the signer's anonymity. In the framework of ring signature, a verifier can be convinced that a signature was produced by an anonymous signer among $n$ possible signers. Here, \textit{anonymity} implies that, for a given signature, it is hard to identify an actual signer whereas the signer exists in $n$ members that each have keys.




Ring signature implies that anyone can check whether it corresponds to a member of the ring but can not know the identity of the actual signer. More formally, a generic digital signature scheme is defined as a set of three PPT algorithms:







\noindent\textbf{Syntax}.

We refer to an ordered list $R = (pk_1, pk_2, \cdots, pk_n)$ of public keys as a ring, and let $R[i] = pk_i$.


\begin{itemize}
  \item $(pk, sk)\gets Ring.KeyGen(1^\lambda)$. It takes as input $1^\lambda$, where $\lambda$ is the security parameter, it produces a pair $(pk, sk)$ of matching public and secret keys.

  \item $Ring.Sign(m, sk_j, \{pk_1, pk_2, \cdots, pk_n \})$. It takes as input different three parameters including: the message $m$, the ring $R$ (or more specific, the set $\{ pk_1, pk_2, \cdots, pk_n \}$ of the public keys of the ring members), and the private key of the signer $sk_j$. Notably, we assume that a user $U_j$ decides to sign a message $m$ on behalf of a ring of users $\{U_1, U_2, \cdots, U_n \}\ni U_j$. Then it outputs a ring signature $\sigma_m$ on message $m$.

  \item $Ring.Vrfy()$. Given a ring signature $\sigma_m$, a message $m$, the set $\{ pk_1, pk_2, \cdots, pk_n \}$ of public keys of the ring members. The boolean function that returns $TRUE$ if the signature is valid and $False$ otherwise. $Vrfy$ is a deterministic algorithm as opposed to probabilistic.
\end{itemize}

Informally, a ring signature scheme is set-up free: The signer does not need the knowledge, consent, or assistance of the other ring members to put them in the ring; all he needs is knowledge of their regular public keys. Different members can use different independent public key signature schemes, with different key and signature sizes. Verification must satisfy the usual soundness and completeness conditions, but in addition we want the signatures to be signer-ambiguous in the sense that a signature should leek no information about the identity of the signer. This anonymity property can be either computational or unconditional.






\noindent\textbf{Correctness}.
Any signature generated by $\Sigma$ must pass the verification test with overwhelming probability.
\href{https://cseweb.ucsd.edu/~smeiklejohn/files/researchexam.pdf}{https://cseweb.ucsd.edu/~smeiklejohn/files/researchexam.pdf}



\href{https://people.csail.mit.edu/rivest/pubs/RST01.pdf}{https://people.csail.mit.edu/rivest/pubs/RST01.pdf}
\noindent\textbf{Security}.





Difference

Below we conclude the main properties of group signature and ring signature.
\begin{itemize}
  \item Group signatures allow any group member to anonymously sign a message on behalf of the group.
  \item Only group managers/issuers are able to add users and trace
or revoke users.
  \item The signatures produced by different group members look indistinguishable to their verifiers, but not to the group manager who can revoke the anonymity of misbehaving signers.
\end{itemize}


We remark that, group signature schemes are often centralized and the group manager has to be a trusted party. The environment of transactions is mostly decentralized. Therefore, ring signatures that are similar to group signatures could be interesting constructions for these decentralized digital services.



\zli{a trusted group manager predefines certain groups of users and distributes specially designed keys to their members. Individual members can then use these keys to anonymously sign messages on behalf of their group. }



\href{https://www.microsoft.com/en-us/research/wp-content/uploads/2017/01/2006-Leak_Secret.pdf}{good servey}








Ring signature is to specify a set of possible signers without revealing which member actually produced the signature. A signer signs a message with a private key and then publishes a set of public keys together with own public key. On the one hand, ring signatures remove the centralization point of a group manager. On the other hand, ring signatures provide a perfect privacy (untracebility) and signer is not able to prove his/her signature (non-repudiation).


Unlike group signatures, we call such signatures ``ring signatures'' instead of ``group signatures'' since rings are geometric regions with uniform periphery and no center.
\begin{itemize}
  \item ring signatures have no group managers, no setup procedures, no revocation procedures, and no coordination: any user can choose any set of possible signers that includes himself, and sign any message by using his secret key and the others' public keys, without getting their approval or assistance.
  \item Ring signatures provide an elegant way to leak authoritative secrets in an anonymous way, to sign casual email in a way that can only be verified by its intended recipient, and to solve other problems in multiparty computations.
\end{itemize}



Same and different

\begin{itemize}
  \item Group signatures are useful when the members want to cooperate, while ring signatures are useful when the members do not want to cooperate.
  \item Both group signatures and ring signatures are signer-ambiguous, but in a ring signature scheme there are no prearranged groups of users, there are no procedures for setting, changing, or deleting groups, there is no way to distribute specialized keys, and there is no way to revoke the anonymity of the actual signer (unless he decides to expose himself).
  \item To produce a ring signature, the actual signer declares an arbitrary set of possible signers that must include himself, and computes the signature entirely by himself using only his secret key and the others’ public keys.
  \item \zli{In cryptography, a ring signature can be performed by any member of a group of users that each have keys. Therefore, a message signed with a ring signature is endorsed by someone in a particular group of people. One of the security properties of a ring signature is that it should be computationally infeasible to determine which of the group members' keys was used to produce the signature. Ring signatures are similar to group signatures but differ in two key ways:
      1) first, there is no way to revoke the anonymity of an individual signature, and 2) second, any group of users can be used as a group without additional setup.}
\end{itemize}


\subsection{Unique Ring Signature}
\par\noindent\textbf{Why we use Unique Ring Signature?}. In our case, a service provider might have the list of public keys that correspond to all users that have purchased a single access to some confidential service for that day (requiring anonymous authentication). For this kind of application, a number of restricted-use ring signatures are proposed. Notable examples include linkable ring signatures~\cite{XXXXX} and traceable ring signatures~\cite{XXXXX}. Both linkable ring signatures and traceable ring signatures admit interesting
applications such as various e-voting systems and e-token systems.


\zli{\href{https://fc13.ifca.ai/proc/5-1.pdf}{https://fc13.ifca.ai/proc/5-1.pdf}}







\par\noindent\textbf{Unique ring signatures}.
Unique ring signatures that capture the essence of linkable ring signatures and traceable ring signatures without identity revelation. \zli{ We may say a ring signature scheme unique if whenever a signer produces two different ring signatures of the same message with respect to the same ring, such that both will pass the verification procedure, then these two ring signatures will always have a large common component (hereinafter unique identifier ).}

For all the applications, we further need a non-colliding property for a unique ring signature. Call a unique ring signature non-colliding if two different signers of the same message, almost never produce ring signatures with the same unique identifier.



\subsubsection{Franklin-Zhang Unique Ring Signature Construction}
\zli{not my invention, just re-write and make it more clear and consistent}
Franklin and Zhang~\cite{FC:FraZha13} inspired by the work of~Bedder, Katz, and Morselli~\cite{JOC:BenKatMor09} and proposed an practical unique ring signature construction in the random oracle mode (ROM). In our setting, we adopt the Franklin-Zhang constriction and apply it XXXXXX.

Below, we highlight their construction. Notably, informally, a ring signature scheme is set-up free: The signer does not need the knowledge, consent, or assistance of the other ring members to put them in the ring. But for to present their algorithm, we introduce a set-up algorithm.

\begin{itemize}
  \item $pp\gets Setup(1^{\lambda})$. The setup algorithm takes as input the security parameter $\lambda$ and outputs a multiplicative group $\bbG$ of prime order $q$ and a randomly chosen generator $g$ of $\bbG$. It also provides two hash functions $\Hsign: \set{0,1}^*\to \bbG$ and $\Hzk: \set{0,1}^*\to \bbZq$. Then it outputs the public parameters (or common reference string) as $pp:=(\secp, q, \bbG, H_0, H_1)$, where $pp$ is posted on the blockchain.

  \item $(pk, sk)\gets KeyGen(1^{\secp}, pp)$. This algorithm is executed by the user $i$ and takes as input the parameter $pp$ and security parameter $\secp$ as input. Then it samples an element $x_i\gets \bbZq$ and sets it as the secret key, i.e., $sk_i:=x_i$. Finally, it computes $y_i\gets g^{x_i}$ and outputs the public key as $pk_i:=y_i=g^{x_i}$.

  \item $\sigma_i \gets Sign(sk_i, R=(pk_1, pk_2, \cdots, pk_n), m)$. This algorithm is executed by the user (i.e., signer) $i$ with the secret key $sk_i=x_i$. In order to sign the message $m$ in the ring $R=\set{pk_i}_1^n=(pk_1, pk_2, \cdots, pk_n)$ for any $i\in [n]$, each signer $i$ acts as the prover and creates an ``or'' composition NIZK-language to prove that a unique identifier $\tau$ (for a message $m$ and a ring $R$) has the same logarithm with respect to base $\Hsign(m \| R)$ as one of the public keys $y_j:= g^{x_j}$ for $j\in [n]$) with respect to base $g$, which can be expressed mathematically as $\log_{\Hsign(m \| R)}{\tau}= \log_{g}{y_i}$ (i.e., $\tau:= \Hsign(m \| R)^{x}=g^x=y$) and the prover knows the witness $x_i$. In particular, the signer $i$ generates the signature in the following ways:
      \begin{enumerate}
        \item User $i$ computes $\tau_i = \Hsign(m \| R)^{x_i}$. Then the users acts as the prover and generates a proof of knowledge of the signature for the statement XXXXXXXXXXX.


        \item For $j\in [n]$ and $j\neq i$, the user (or prover in NIZK) selects $c_j, t_j\gets \bbZq$ for (Pedersen) commitment and computes %$a_j= g^{t_i}y_j^{c_j}=g^{t_i}(g^{x_j})^{c_j}$ and $b_j=\Hsign(m \| R)^{t_i} (\Hsign(m \| R)^{x_j})^{c_j}$.
            \begin{eqnarray*}
            % \nonumber to remove numbering (before each equation)
              a_j &=& g^{t_i}y_j^{c_j}=g^{t_i}(g^{x_j})^{c_j}, \\
              b_j &=& \Hsign(m \| R)^{t_i} (\Hsign(m \| R)^{x_j})^{c_j}.
            \end{eqnarray*}






        \item For $j=i$, the user (or prover in NIZK)  selects $r_i\gets \bbZq$ and computes %$a_i\gets g^{r_i}$ and $b_i\gets \Hsign(m \| R)^{r_i}$.
            \begin{eqnarray*}
            % \nonumber to remove numbering (before each equation)
              a_i &=& g^{r_i}, \\
              b_i &=& \Hsign(m \| R)^{r_i}.
            \end{eqnarray*}






        \item Computes $\bar{c}\gets\Hzk(m, R, \set{a_j, b_j}_1^n)$ and obtains the challenge $c_i=\bar{c}-\sum_{i\neq j} c_j\pmod{q}$ for NIZK, then generates the proof of correctness $\pi_i= r_i -c_i\cdot x_i$ with the witness $x_i$ and its associated masking $r_i$, then the user (or prover in NIZK) sends the set of challenge-proof pairs $\set{(c_i, \pi_i)}_1^n$ to the verifier. Meanwhile, the user (or prover in NIZK) also sends the masking statements $\set{a_j, b_j}_1^n$ to the verifier.
      \end{enumerate}
      Finally, user $i$ generates the signature $\sigma_i=(\tau_i, \set{c_i, \pi_i}_1^n)$, and outputs
       $$(R, m, \sigma_i=(\tau_i=\Hsign(m\| R)^{x_i}, \set{c_i, \pi_i}_1^n)).$$

      \item $Vrfy(sk, m, \sigma_i)$. Upon receiving the signature $(R, m, \sigma_m)$, the verification algorithm first parses $\sigma_m$ as
          $(\tau, (c_1, \pi_1), (c_2, \pi_2), \cdots, (c_n, \pi_n))$ and checks whether
          \begin{equation*}
            \sum_1^n c_j = \Hzk(m, R, \set{ \underline{g^{\pi_j}y_j^{c_j}}, \underline{H(m\|R)^{\pi_j} \tau^{c_j}}   }_1^n).
          \end{equation*}
          Namely, checks $a_j\overset{?}{=}g^\pi y^c$ and $b_j \overset{?}{=} H(m\|R)^\pi \tau^c$ for $\pi=r-cx$.

          %where $g^r\overset{?}{=}g^\pi y^c$ and $\Hsign(m)^r \overset{?}{=} H(m\|R)^\pi \tau^c$ for $\pi=r-cx$.

\end{itemize}


%\begin{theorem}
The scheme is a unique ring signature in the random oracle under the Decisional Diffie–Hellman assumption.
%\end{theorem}


\par\noindent\textbf{Uniqueness}.
The signature should have the form of




\zli{If unique signature is not necessary, so we can follow AC17 Mlavola-Schr{\"{o}}der~\cite{AC:MalSch17}}

and \href{https://eprint.iacr.org/2019/135.pdf}{ePrint2019/135}
and \href{https://www.microsoft.com/en-us/research/wp-content/uploads/2017/01/2006-Leak_Secret.pdf}{How to Leak a Secret}










\zli{We do not need group signature}
\subsection{(Anonymous) Dynamic Group Signature}
\zli{
\href{https://cseweb.ucsd.edu/~mihir/papers/bsz.pdf}{https://cseweb.ucsd.edu/~mihir/papers/bsz.pdf}
with the concrete construction \href{https://eprint.iacr.org/2016/154.pdf}{https://eprint.iacr.org/2016/154.pdf}. More practical, we can refer to \href{https://crypto.stanford.edu/~dabo/pubs/papers/groupsigs.pdf}{https://crypto.stanford.edu/~dabo/pubs/papers/groupsigs.pdf}
}
A dynamic group signature scheme involves a \textit{trusted party} who generates the initial keys, an authority named \textit{issuer}, an authority named \textit{opener} and a set of \textit{users} who are potential group members.

\noindent\textbf{Syntax}. The scheme $\Pi_{GS}$ consists of the following PPT algorithms.
\begin{itemize}
  \item[-] $(gpk, ik, ok) \gets GGen(1^{\lambda})$. This algorithm is executed by the trusted party given the security parameter $\lambda$ and outputs a triple $(gpk, ik, ok)$, where the \textit{issue key} is given to the \textit{issuer}, the \textit{opening key} is given to the \textit{opener}, and the \textit{group public key} is make public as common string reference (or CRS).
  \item[-] $(upk, usk) \gets UGen(1^{\lambda})$. This algorithm is executed by the user who intends to be a group member given the security parameter $\lambda$. Then it outputs a personal key pair $(upk, usk)$, where we assume the \textit{user public key} $upk$ is public.

  \item[-] $(gsk, reg[i])\gets\inner{Join, Issue}$. This is an interactive group-joining protocol executed by the issuer and a user.  If it completes successfully, the issuer registers this user to the group and this user becomes a group member. Importantly, the final state of the $Join$ is denoted by the \textit{group secret signing key} $gsk$ while the final state of the $Iss$ is denoted to the registration information $reg[i]$ stored in the registration table $reg$.

      \begin{itemize}
        \item[-] $Join(gpk, usk_i, upk_i)$.
        \item[-] $Issue(gpk, ik, i, upk_i, reg)$.
      \end{itemize}



      \zli{If we don't require the user can dynamically join the group, the dynamic group signature can decrease to traditional group signature.}


  \item $\sigma_{msg} \gets Sign(gpk, gsk_i, msg)$. This algorithm is executed by the group member (i.e., user $i$), then outputs a signature $\sigma_{msg}$ corresponding to the message $msg\in \set{0,1}^*$ under the group signing key $gsk_i$.

  \item $\set{0,1} \gets Vrfy(gpk, msg, \sigma_{msg})$. This algorithm outputs a bit $b\in \set{0,1}$ indicating whether or not $\sigma_{msg}$ is a valid signature on message $msg$, with respect to the group public key $gpk$.


  \item $(i, \pi_{open})\gets Open(gpk,ok, reg, msg, \sigma_{msg})$. This algorithm is executed by the opener who has the read-access to the registration table $reg$, finally, the opener can extract the identity of the signer $i$ with the corresponding proof $\pi_{open}$, then outputs a pair $(i, \pi_{open})$. \zli{this is the reason why we need ZKP}


  \item $\set{0,1}\gets Judge(gpk, msg, \sigma_{msg}, i, upk_i, \pi_{open})$. This algorithm outputs  a bit $b\in \set{0,1}$ to check whether or not $\pi_{open}$ is a proof that the user (or index) $i$ produced the valid signature $\sigma_{msg}$, with respect to the group public key $gpk$ and message $msg$.

  \end{itemize}

\noindent\textbf{Correctness}. In a nutshell, correctness requires that for any signature generated by honest group members, the following should hold: the signature should be valid; the opening algorithm, given the message and signature, should correctly identify the signer; the proof returned by the opening algorithm should be accepted by the judge.




\noindent\textbf{Security}.


\noindent\textbf{Properties}.
\begin{itemize}
  \item \textbf{Traceability} requires that every valid signature should be traced to some group member and the opener is able to generate a proof accepted by the judge.
  \item \textbf{Full Anonymity} requires that it is infeasible to recover the identity of a signer from a signature, even if the adversary is given access to the opening oracle.
  \item \textbf{Non-frameability} requires that the adversary is unable to generate a proof, which is accepted by the judge, that an honest user generated a valid signature unless this user really did generate this signature.
\end{itemize}





\par\noindent\textbf{Linkable ring signatures}. Linkable ring signature asks that if a user signs any two messages (same or different) with respect to the same ring, then an efficient public procedure can verify that the signer was the same (although the user’s identity is not revealed).
\href{https://eprint.iacr.org/2019/654.pdf}{ePrint2019/654}
\href{https://eprint.iacr.org/2018/728.pdf}{ePrint2018/728}


\zli{ The property of linkability allows one to determine whether any two signatures have been produced by the same member (under the same private key). The identity of the signer is nevertheless preserved. One of the possible applications can be an offline e-cash system.}




\par\noindent\textbf{Traceable ring signatures}. In traceable ring signatures,
each message is signed not only with respect to a list of ring members, but also with respect to an issue (e.g., identifying label of a specific election or survey). If a user signs any two different messages with respect to the same list of ring members and the same issue label, then the user’s identity is revealed by an efficient public procedure. If a user signs the same message twice with respect to the same list of ring members and the same issue label, then the two signed messages can be determined to have come from the same signer by an efficient public procedure (although the signer’s identity remains concealed)


\zli{ the public key of the signer is revealed (if they issue more than one signatures under the same private key)}





==> sec/related.tex <==
\section{Related Work}
\label{sec:related}
We have discussed related work extensively in the previous sections. Here, we highlight two orthogonal research
directions that may benefit from our work. First, off-chain scaling systems such as Plasma~\cite{plasma} and sidechains~\cite{sidechain} use multiple blockchains to improve overall throughput. Our work can be applied to
make communication between the sub-chains more efficient and richer. Second, there is a trend towards
decentralized systems, of which blockchain is only one example. Other examples include identity
management~\cite{coniks}, personal storage~\cite{upspin}, and social network~\cite{decent}. These systems
exist in silos, and our work can be applied to build novel applications on top of them. 

